Ties at the Top: A Point-in-Time Comparison of CVSS and EPSS at a Fixed Budget

Organizations must decide which vulnerabilities warrant further analysis and protective action when the volume of published vulnerabilities exceeds their analytical capacity. We present a methodology for comparing vulnerability-prioritization strategies under an explicit resource constraint, represented by a fixed number of CVEs selected from a common eligible population. We apply this methodology to the Common Vulnerability Scoring System (CVSS) and the Exploit Prediction Scoring System (EPSS). For CVEs published in the National Vulnerability Database (NVD) from 17 March to 31 December 2025 and from 1 January to 31 March 2026 (Q1), we reconstruct each CVE's scores and status 30 days after NVD publication, using archived source data. Each cohort has one ranking per strategy at a 5% budget. Positives are CVEs added to the Known Exploited Vulnerabilities (KEV) catalog within 180 days after their decision day. The catalog is maintained by the Cybersecurity and Infrastructure Security Agency (CISA). EPSS captures 16 of 40 positives in 2025, versus 5 for CVSS; alternative selections among tied CVEs cannot raise CVSS capture above 9. In Q1, CVSS captures 4 of 11 and EPSS 3, but tie-breaking can reverse this ordering. The score alone leaves most of each CVSS list undecided: the tie-breaking rule allocates 1,678 of 1,919 CVSS places in 2025 and 589 of 758 in Q1 among CVEs tied at score 9.8. Most chosen CVSS scores come from non-NVD providers; disabling those scores reduces CVSS capture from 5 to 1 in 2025 and from 4 to 0 in Q1. A fixed-budget comparison should therefore report its decision cutoff, eligible population, score provenance, and tie-breaking rule.

==> sections/author_typography.tex <==
\makeatletter
% Keep author names plain and display their full ORCID identifiers as links.
\renewcommand{\orcid}[1]{%
  \unskip\ignorespaces
  \expandafter\gdef\csname typeset@author\the\num@authors\endcsname##1{%
    ##1\nobreakspace{\normalfont\rmfamily\fontsize{9}{10.8}\selectfont
      \href{https://orcid.org/#1}{(ORCID: #1)}}}}
\patchcmd{\institution}{\unskip~}{\unskip}{}{\PackageError{author-layout}{Affiliation alignment patch failed}{}}
\renewcommand{\@authorfont}{\normalfont\rmfamily\fontsize{12}{14.4}\selectfont}
\renewcommand{\@affiliationfont}{\normalfont\rmfamily\fontsize{10}{12}\selectfont}
\patchcmd{\@mkauthors@i}{\MakeUppercase}{\@firstofone}{}{\PackageError{author-layout}{Author style patch failed}{}}
\patchcmd{\@mkauthors@i}{\MakeUppercase}{\@firstofone}{}{\PackageError{author-layout}{Author style patch failed}{}}
\renewcommand{\@typeset@author@line}{%
  \andify\@currentauthors\par\noindent
  \@currentauthors\def\@currentauthors{}%
  \ifx\@currentaffiliations\@empty\else
    \andify\@currentaffiliations
    \par\noindent{\@currentaffiliations}\par
  \fi
  \def\@currentaffiliations{}}
\apptocmd{\@mkauthors@i}{%
  \global\setbox\mktitle@bx=\vbox{\unvbox\mktitle@bx\vskip4pt}%
}{}{\PackageError{author-layout}{Author spacing patch failed}{}}
\makeatother

